$\psi$-Epistemic Models, Einsteinian Intuitions, and No-Gos. A Critical Study of Recent Developments on the Quantum State

Quantum mechanics notoriously faces the measurement problem, the problem that if read thoroughly, it implies the nonexistence of definite outcomes in measurement procedures. A plausible reaction to this and to related problems is to regard a system's quantum state $|\psi\rangle$ merely as an indication of our lack of knowledge about the system, i.e., to interpret it epistemically. However, there are radically different ways to spell out such an epistemic view of the quantum state. We here investigate recent developments in the branch that introduces hidden variables $\lambda$ in addition to the quantum state $|\psi\rangle$ and has its roots in Einstein's views. In particular, we confront purported achievements of a concrete model that has been considered to serve as evidence for an epistemic view of the envisioned kind, as well as specific no-go results and their import. It will be argued that while an epistemic account of the particular kind is not straightforwardly ruled out by the no-go results, they demonstrate that the evidential character of the model(s) discussed rests on a rather shaky foundation, and that they make some achievements widely recognized in the literature appear worthy of doubt.

==> bbm/README <==
Copyright 1993 Gilles F. Robert.
You may freely use, modify and/or distribute this file.
This statement added 2008/11/14 by Clea F. Rees on the basis of the email exchange archived at http://lists.debian.org/debian-tex-maint/2008/05/msg00040.html.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A mathematician often needs special symbols to designate sets such as the
integers, the reals etc..

For the time being, the only fonts providing these special symbols have been:
 - the AMS fonts msbm (older version msym), which are intended for use with
Times and aren't truly what a mathematician expects (the stress is on both
stems instead of being on only the left one).
 - Alan Jeffrey's bbold fonts, which are sans-serif ones, with (almost) no
possibility of design variations for, say, a bold variant.
That was all, and in particular nothing for use with Computer Modern.

I was already working at that time on the project of changing the codes of
romanu.mf, romanl.mf and other files to add a 'Blackboard' variant to
Computer Modern.

                YOU HAVE IT ALL THERE !!!

The whole package contains five 'main' files:
 - blbbase.mf (the 'base') contains the supplementary definitions needed
for double stems etc..
 - blbord.mf (the 'driver') is fairly simple and only makes the necessary
calls.
 - blbordu.mf (based on romanu.mf): programs for uppercase letters.
 - blbordl.mf (based on romanl.mf): programs for lowercase letters.
 - blbordsp.mf (based on romand.mf and punct.mf): programs for the digits~1
and~2 and for parentheses and brackets.

There is also a whole lot of parameter files that are (almost) the same as
those provided by DEK.

For most of them, the only differences are
- change 'cmbase' for 'blbbase' on line~2
- change 'generate roman' for 'generate blbord' on last line
- add two extra parameters (interspace# and cap_interspace#).

A LaTeX(2e) package written by Torsten Hilbrich for using these fonts is also 
available nearby, exactly in ctan/macros/latex/contrib/supported/bbm/

I sincerely hope you'll enjoy using these fonts; if you get into problems
while using them, I should be reachable at

 _ _       Gilles F. ROBERT
|          Unit\'e de Math\'ematiques Pures et Appliqu\'ees
|  _ _ _   \'Ecole Normale Sup\'erieure
|   |   |  46, All\'ee d'Italie
|_ _|_ _|  69364 Lyon Cedex (FRANCE)
    |  \
    |   \  e-mail : gfrobert@umpa.ens-lyon.fr

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> bbm/test.tex <==
% Copyright 1993 Gilles F. Robert.
% You may freely use, modify and/or distribute this file.
% This statement added 2008/11/14 by Clea F. Rees on the basis of the email exchange archived at http://lists.debian.org/debian-tex-maint/2008/05/msg00040.html.
%
\let\noinit!\input testfont
\def\fontname{bbm17 }\startfont\table
\def\fontname{bbm12 }\startfont\table
\eject
\def\fontname{bbm10 }\startfont\table
\def\fontname{bbm9 }\startfont\table
\eject
\def\fontname{bbm8 }\startfont\table
\def\fontname{bbm7 }\startfont\table
\eject
\def\fontname{bbm6 }\startfont\table
\def\fontname{bbm5 }\startfont\table
\eject
\def\fontname{bbmsl12 }\startfont\table
\def\fontname{bbmsl10 }\startfont\table
\eject
\def\fontname{bbmsl9 }\startfont\table
\def\fontname{bbmsl8 }\startfont\table
\eject
\def\fontname{bbmbx12 }\startfont\table
\def\fontname{bbmbx10 }\startfont\table
\eject
\def\fontname{bbmbx9 }\startfont\table
\def\fontname{bbmbx8 }\startfont\table
\eject
\def\fontname{bbmbx7 }\startfont\table
\def\fontname{bbmbx6 }\startfont\table
\eject
\def\fontname{bbmbx5 }\startfont\table
\def\fontname{bbmbxsl10 }\startfont\table
\eject
\def\fontname{bbmss17 }\startfont\table
\def\fontname{bbmss12 }\startfont\table
\eject
\def\fontname{bbmss10 }\startfont\table
\def\fontname{bbmss9 }\startfont\table
\eject
\def\fontname{bbmss8 }\startfont\table
\def\fontname{bbmssq8 }\startfont\table
\eject
\def\fontname{bbmssi17 }\startfont\table
\def\fontname{bbmssi12 }\startfont\table
\eject
\def\fontname{bbmssi10 }\startfont\table
\def\fontname{bbmssi9 }\startfont\table
\eject
\def\fontname{bbmssi8 }\startfont\table
\def\fontname{bbmssqi8 }\startfont\table
\eject
\def\fontname{bbmssbx10 }\startfont\table
\def\fontname{bbmssdc10 }\startfont\table
\eject
\def\fontname{bbmtt12 }\startfont\table
\def\fontname{bbmtt10 }\startfont\table
\eject
\def\fontname{bbmtt9 }\startfont\table
\def\fontname{bbmtt8 }\startfont\table
\eject
\def\fontname{bbmsltt10 }\startfont\table
\def\fontname{bbmvtt10 }\startfont\table
\eject
\def\fontname{bbmb10 }\startfont\table
\def\fontname{bbmfib8 }\startfont\table
\eject
\def\fontname{bbmdunh10 }\startfont\table
\bye


==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

